The Duo of Artificial Intelligence and Big Data for Industry 4.0: Review of Applications, Techniques, Challenges, and Future Research Directions

The increasing need for economic, safe, and sustainable smart manufacturing combined with novel technological enablers, has paved the way for Artificial Intelligence (AI) and Big Data in support of smart manufacturing. This implies a substantial integration of AI, Industrial Internet of Things (IIoT), Robotics, Big data, Blockchain, 5G communications, in support of smart manufacturing and the dynamical processes in modern industries. In this paper, we provide a comprehensive overview of different aspects of AI and Big Data in Industry 4.0 with a particular focus on key applications, techniques, the concepts involved, key enabling technologies, challenges, and research perspective towards deployment of Industry 5.0. In detail, we highlight and analyze how the duo of AI and Big Data is helping in different applications of Industry 4.0. We also highlight key challenges in a successful deployment of AI and Big Data methods in smart industries with a particular emphasis on data-related issues, such as availability, bias, auditing, management, interpretability, communication, and different adversarial attacks and security issues. In a nutshell, we have explored the significance of AI and Big data towards Industry 4.0 applications through panoramic reviews and discussions. We believe, this work will provide a baseline for future research in the domain.

==> Backup.tex <==
\subsubsection{Security in IIoT Ecosystem}

Physical world integration with cyber world opens the opportunity of creating smart environments; this new paradigm is called the Internet of Things (IoT). Communication between humans and objects has been extended into those between objects and objects. Industrial IoT (IIoT) takes benefits of IoT communications in business applications focusing in interoperability between machines (i.e., IIoT is a subset from the IoT). Number of daily life things and objects connected to the Internet has been in increasing fashion, which makes the IoT be the dynamic network of networks. Challenges such as heterogeneity, dynamicity, velocity, and volume of data, make IoT services produce inconsistent, inaccurate, incomplete, and incorrect results, which are critical for many applications especially in IIoT (e.g., health-care, smart transportation, wearable, finance, industry, etc.). Discovering, searching, and sharing data and resources reveal 40\% of IoT benefits to cover almost industrial applications. Enabling real-time data analysis, knowledge extraction, and search techniques based on Information Communication Technologies (ICT), such as data fusion, machine learning, big data, cloud computing, blockchain, etc., can reduce and control IoT and leverage its value. This research presents a comprehensive review to study state-of-the-art challenges and recommended technologies for enabling data analysis and search in the future IoT presenting a framework for ICT integration in IoT layers. This paper surveys current IoT search engines (IoTSEs) and presents two case studies to reflect promising enhancements on intelligence and smartness of IoT applications due to ICT integration.
\cite{younan_challenges_2020} \par

In the past 10 years, ubiquitous manufacturing (UM) has received a growing amount of attention among researchers in the manufacturing community because ubiquitous computing technologies (UCTs) can be applied to address a wide range of issues in the manufacturing industry, e.g. manufacturing processes and equipment, manufacturing management and planning. However, to the best of the authors’ knowledge, there is a lack of comprehensive and critical review from a holistic view of the state-of-the-art UM and its systems. This paper aims to provide a concise overview of the technical features, characteristics and broad range of applications of UM systems published between 1997 and 2017. Among these selected articles, more than 70\% of them were published between 2012 and 2017, and they are considered as recent pertinent works which will be discussed in detail. The unique aspects of this paper lie in that this paper summarises and analyses a broad range of the state-of-the-art implementation of UM systems from a holistic and comprehensive view of manufacturing technology, including UM for manufacturing processes, manufacturing control systems, logistics, remanufacturing, cloud manufacturing, production scheduling, production quality control and evaluation, etc. In addition, the current limitation factors and future trends of UM development will also be discussed.
\cite{wang_comprehensive_2018} \par

A new industrial revolution is undergoing, based on a number of technological paradigms. The will to foster and guide this phenomenon has been summarized in the expression “Industry 4.0” (I4.0). Initiatives under this term share the vision that many key technologies underlying Cyber-Physical Systems and Big Data Analytics are converging to a new distributed, highly automated, and highly dynamic production network, and that this process needs regulatory and cultural advancements to effectively and timely develop. In this work, we focus on the technological aspect only, highlighting the unprecedented complexity of I4.0 emerging from the scientific literature. While previous works have focused on one or up to four related enablers, we consider ten technological enablers, including besides the most cited Big Data, Internet of Things, and Cloud Computing, also others more rarely considered as Fog and Mobile Computing, Artificial Intelligence, Human-Computer Interaction, Robotics, down to the often overlooked, very recent, or taken for granted Open-Source Software, Blockchain, and the Internet. For each we explore the main characteristics in relation to I4.0 and its interdependencies with other enablers. Finally we provide a detailed analysis of challenges in leveraging each of the enablers in I4.0, evidencing possible roadblocks to be overcome and pointing at possible future directions of research. Our goal is to provide a reference for the experts in some of the technological fields involved, for a reconnaissance of integration and hybridization possibilities with other fields in the endeavor of I4.0, as well as for the laymen, for a high-level grasp of the variety (and often deep history) of the scientific research backing I4.0.
\cite{aceto_survey_2019} \par

Artificial intelligence, big data, machine learning, cloud computing, and Internet of Things (IoT) are terms which have driven the fourth industrial revolution. The digital revolution has transformed the manufacturing industry into smart manufacturing through the development of intelligent systems. In this paper, a big data ecosystem is presented for the implementation of fault detection and diagnosis in predictive maintenance with real industrial big data gathered directly from large-scale global manufacturing plants, aiming to provide a complete architecture which could be used in industrial IoT-based smart manufacturing in an industrial 4.0 system. The proposed architecture overcomes multiple challenges including big data ingestion, integration, transformation, storage, analytics, and visualization in a real-time environment using various technologies such as the data lake, NoSQL database, Apache Spark, Apache Drill, Apache Hive, OPC Collector, and other techniques. Transformation protocols, authentication, and data encryption methods are also utilized to address data and network security issues. A MapReduce-based distributed PCA model is designed for fault detection and diagnosis. In a large-scale manufacturing system, not all kinds of failure data are accessible, and the absence of labels precludes all the supervised methods in the predictive phase. Furthermore, the proposed framework takes advantage of some of the characteristics of PCA such as its ease of implementation on Spark, its simple algorithmic structure, and its real-time processing ability. All these elements are essential for smart manufacturing in the evolution to Industry 4.0. The proposed detection system has been implemented into the real-time industrial production system in a cooperated company, running for several years, and the results successfully provide an alarm warning several days before the fault happens. A test case involving several outages in 2014 is reported and analyzed in detail ...
\cite{yu_global_2020} \par

Manufacturing and service organisations improve their processes on a continuous basis to have better operational performance. They use lean six sigma (LSS) projects for process improvement. Therefore, this study aims to investigate the existing literature in LSS and the application of big data analytics (BDA) to have more confident and predictable decisions in each phase of LSS. Fifty-two articles have been identified after a careful and vigilant screening of closely related themes. Future research directions in the big data and LSS have been highlighted on the basis of organisational theories. Review presents an investigation framework consisting of BDA techniques applicable to each phase of LSS in all the dimensions such as volume, variety, velocity and veracity of big data. Review highlights the concerns of big data in LSS such as system design and integration, system performance, security and reliability of data, sustaining the control and conducting the experiments, distributed material and information flow. The review unveils the application of 8 modern organisational theories to big data in LSS with 21 key aspects of related theories and 19 distinct research gaps as opportunities for future research.
\cite{gupta_big_2020} \par

Edge Computing represents the activities of IoT (Internet of Things) devices at the border or limit of the network connected to the remote Cloud. The latest research in this field has intended to demonstrate that Edge Computing architectures are the optimal solution to minimising latency, improving privacy and reducing bandwidth costs in IoT-based scenarios. This article is a review of the Edge Computing technology and its reference architectures proposed by the Edge Computing Consortium, Intel-SAP, the FAR-Edge Project and the Industrial Internet Consortium for Industry 4.0. Moreover, this article presents a proposal for a tiered architecture with a modular approach that allows to manage the complexity of solutions not only for Industry 4.0 environments but also for other scenarios such as smart cities, smart energy, healthcare or precision agrotechnology. The main contributions of the proposed architecture reside in the security and privacy provided by blockchain technologies. Finally, the proposed reference architecture is tested by building an IoT platform in a smart agroindustry scenario to reduce bandwidth costs between the Edge and the Cloud.
\cite{sitton-candanedo_review_2019} \par

The healthcare industry has revolutionized from 1.0 to 4.0 where Healthcare 1.0 was more doctor centric and Healthcare 2.0 replaced manual records with electronic healthcare records (EHRs). Healthcare 3.0 was patient-centric and Healthcare 4.0 uses cloud computing (CC), fog computing (FC), Internet of things (IoT), and telehealthcare technologies to share data between various stakeholders. However, framing a secure technique for Healthcare 4.0 has always been a challenging task. An in-secure technique for Healthcare 4.0 may lead to the healthcare data breach where hackers can gain full access to patients’ email accounts, messages, and reports. On the contrary, a secured technique for Healthcare 4.0 can provide satisfaction to all stakeholders, including patients and caregivers. Motivated from these facts, this paper presents an extensive literature review and analysis of state-of-the-art proposals to maintain security and privacy in Healthcare 4.0. We also explored the blockchain-based solution to give insights to both researchers and practitioners communities. Different taxonomies used for exploring various security and privacy issues in Healthcare 4.0 are also presented in a structured manner. Then, the advantages and limitations of various security and privacy techniques are explored and discussed in the paper. Finally, existing challenges and future research directions of security and privacy in Healthcare 4.0 are presented.
\cite{hathaliya_exhaustive_2020} \par

The adoption of emerging technological trends and applications of the Internet of Things (IoT) in the industrial systems is leading towards the development of Industrial IoT (IIoT). IIoT serves as a new vision of IoT in the industrial sector by automating smart objects for sensing, collecting, processing and communicating the real-time events in industrial systems. The major objective of IIoT is to achieve high operational efficiency, increased productivity, and better management of industrial assets and processes through product customization, intelligent monitoring applications for production floor shops and machine health, and predictive and preventive maintenance of industrial equipment. In this paper, we present a new and clear definition of IIoT, which can help the readers to understand the concept of IIoT. We have described the state-of-the-art research efforts in IIoT. Finally, we have highlighted the enabling technologies for IIoT and recent challenges faced by IIoT.
\cite{khan_industrial_2020} \par

Wireless sensor networks (WSNs) have evolved to become an integral part of the contemporary Internet of Things (IoT) paradigm. The sensor node activities of both sensing phenomena in their immediate environments and reporting their findings to a centralized base station (BS) have remained a core platform to sustain heterogeneous service-centric applications. However, the adversarial threat to the sensors of the IoT paradigm remains significant. Denial of service (DoS) attacks, comprising a large volume of network packets, targeting a given sensor node(s) of the network, may cripple routine operations and cause catastrophic losses to emergency services. This paper presents an intelligent DoS detection framework comprising modules for data generation, feature ranking and generation, and training and testing. The proposed framework is experimentally tested under actual IoT attack scenarios, and the accuracy of the results is greater than that of traditional classification techniques.
\cite{baig_averaged_2020} \par


\subsubsection{Privacy in IIoT Cloud Services}
Applications of Blockchain (BC) technology and Cyber-Physical Systems (CPS) are increasing exponentially. However, framing resilient and correct smart contracts (SCs) for these smart application is a quite challenging task because of the complexity associated with them. SC is modernizing the traditional industrial, technical, and business processes. It is self-executable, self-verifiable, and embedded into the BC that eliminates the need for trusted third-party systems, which ultimately saves administration as well as service costs. It also improves system efficiency and reduces the associated security risks. However, SCs are well encouraging the new technological reforms in Industry 4.0, but still, various security and privacy challenges need to be addressed. In this paper, a survey on SC security vulnerabilities in the software code that can be easily hacked by a malicious user or may compromise the entire BC network is presented. As per the literature, the challenges related to SC security and privacy are not explored much by the authors around the world. From the existing proposals, it has been observed that designing a complex SCs cannot mitigate its privacy and security issues. So, this paper investigates various Artificial Intelligence (AI) techniques and tools for SC privacy protection. Then, open issues and challenges for AI-based SC are analyzed. Finally, a case study of retail marketing is presented, which uses AI and SC to preserve its security and privacy.
\cite{Smart Contract Privacy Protection Using AI in Cyber-Physical Systems: Tools, Techniques and Challenges}\par 

By leveraging deep learning-based technologies, industrial artificial intelligence (IAI) has been applied to solve various industrial challenging problems in Industry 4.0. However, for privacy reasons, traditional centralized training may be unsuitable for sensitive data-driven industrial scenarios, such as healthcare and autopilot. Recently, federated learning has received widespread attention, since it enables participants to collaboratively learn a shared model without revealing their local data. However, studies have shown that, by exploiting the shared parameters adversaries can still compromise industrial applications such as auto-driving navigation systems, medical data in wearable devices, and industrial robots’ decision making. In this article, to solve this problem, we propose an efficient and privacy-enhanced federated learning (PEFL) scheme for IAI. Compared with existing solutions, PEFL is noninteractive, and can prevent private data from being leaked even if multiple entities collude with each other. Moreover, extensive experiments with real-world data demonstrate the superiority of PEFL in terms of accuracy and efficiency.
\cite{Efficient and Privacy-enhanced Federated Learning for Industrial Artificial Intelligence} \par 

Context: A fog computing architecture that is geographically distributed and to which a variety of heterogeneous devices are ubiquitously connected at the end of a network in order to provide collaboratively variable and flexible communication, computation, and storage services. Fog computing has many advantages and it is suited for the applications whereby real-time, high response time, and low latency are of the utmost importance, especially healthcare applications. Objectives: The aim of this study was to present a systematic literature review of the technologies for fog computing in the healthcare IoT systems field and analyze the previous. Providing motivation, limitations faced by researchers, and suggestions proposed to analysts for improving this essential research field. Methods: The investigations were systematically performed on fog computing in the healthcare field by all studies; furthermore, the four databases Web of Science (WoS), ScienceDirect, IEEE Xplore Digital Library, and Scopus from 2007 to 2017 were used to analyze their architecture, applications, and performance evaluation. Results: A total of 99 articles were selected on fog computing in healthcare applications with deferent methods and techniques depending on our inclusion and exclusion criteria. The taxonomy results were divided into three major classes; frameworks and models, systems (implemented or architecture), review and survey. Discussion: Fog computing is considered suitable for the applications that require real-time, low latency, and high response time, especially in healthcare applications. All these studies demonstrate that resource sharing provides low latency, better scalability, distributed processing, better security, fault tolerance, and privacy in order to present better fog infrastructure. Learned lessons: numerous lessons related to fog computing. Fog computing without a doubt decreased latency in contrast to cloud computing. Researchers show that simulation and experimental proportions ensure substantial reductions of latency is provided. Which it is very important for healthcare IoT systems due to real-time requirements. Conclusion: Research domains on fog computing in healthcare applications differ, yet they are equally important for the most parts. We conclude that this review will help accentuating research capabilities and consequently expanding and making extra research domains.
\cite{Enabling technologies for fog computing in healthcare IoT systems}

Industrial cyber-physical systems are the primary enabling technology for Industry 4.0, which combine legacy industrial and control engineering, with emerging technology paradigms (e.g. big data, internet-of-things, artificial intelligence, and machine learning), to derive self-aware and self-configuring factories capable of delivering major production innovations. However, the technologies and architectures needed to connect and extend physical factory operations to the cyber world have not been fully resolved. Although cloud computing and service-oriented architectures demonstrate strong adoption, such implementations are commonly produced using information technology perspectives, which can overlook engineering, control and Industry 4.0 design concerns relating to real-time performance, reliability or resilience. Hence, this research compares the latency and reliability performance of cyber-physical interfaces implemented using traditional cloud computing (i.e. centralised), and emerging fog computing (i.e. decentralised) paradigms, to deliver real-time embedded machine learning engineering applications for Industry 4.0. The findings highlight that despite the cloud’s highly scalable processing capacity, the fog’s decentralised, localised and autonomous topology may provide greater consistency, reliability, privacy and security for Industry 4.0 engineering applications, with the difference in observed maximum latency ranging from 67.7\%–99.4\%. In addition, communication failures rates highlighted differences in both consistency and reliability, with the fog interface successfully responding to 900,000 communication requests (i.e. 0\% failure rate), and the cloud interface recording failure rates of 0.11\%, 1.42\%, and 6.6\% under varying levels of stress.
\cite{A comparison of fog and cloud computing cyber-physical interfaces for Industry 4.0 real-time embedded machine learning engineering applications}

Internet of Things (IoT) is a term that has been introduced in recent years, and it defines objects being able to connect and transfer data through the internet. Although some IoT-related products are currently available in the market, there are still some IoT problems that need to be overcome, such as the security issues and lack of confidence and understanding of IoT. This study aims to analyze the influential factors in building successful IoT system for IoT-related enterprises. This study develops a rule-based decision support mechanism using fuzzy set theory and the Analytic Hierarchy Process (AHP) to evaluate the influential factors in IoT. This study finds that tangible factors (Security, Value and Connectivity) are more important than the intangible factors (Telepresence and Intelligence). Finally, this study concludes that after enterprises build a good IoT connectivity system, it is essential to combine this with good IoT security to create a successful IoT environment. Enterprises should also consider both IoT security and IoT values for the IoT products and employees' working convenience.
\cite{Fuzzy AHP analysis of Internet of Things (IoT) in enterprises}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%....Impact  of  5G  and  Wireless  services  in  Modern  Indus-tries:

The increasing consumption of multimedia services and the demand of high-quality services from customers has triggered a fundamental change in how we administer networks in terms of abstraction, separation, and mapping of forwarding, control and management aspects of services. The industry and the academia are embracing 5G as the future network capable to support next generation vertical applications with different service requirements. To realize this vision in 5G network, the physical network has to be sliced into multiple isolated logical networks of varying sizes and structures which are dedicated to different types of services based on their requirements with different characteristics and requirements (e.g., a slice for massive IoT devices, smartphones or autonomous cars, etc.). Softwarization using Software-Defined Networking (SDN) and Network Function Virtualization (NFV)in 5G networks are expected to fill the void of programmable control and management of network resources.
In this paper, we provide a comprehensive review and updated solutions related to 5G network slicing using SDN and NFV. Firstly, we present 5G service quality and business requirements followed by a description of 5G network softwarization and slicing paradigms including essential concepts, history and different use cases. Secondly, we provide a tutorial of 5G network slicing technology enablers including SDN, NFV, MEC, cloud/Fog computing, network hypervisors, virtual machines & containers. Thidly, we comprehensively survey different industrial initiatives and projects that are pushing forward the adoption of SDN and NFV in accelerating 5G network slicing. A comparison of various 5G architectural approaches in terms of practical implementations, technology adoptions and deployment strategies is presented. Moreover, we provide a discussion on various open source orchestrators and proof of concepts representing industrial contribution. The work also investigates the standardization efforts in 5G networks regarding network slicing and softwarization. Additionally, the article presents the management and orchestration of network slices in a single domain followed by a comprehensive survey of management and orchestration approaches in 5G network slicing across multiple domains while supporting multiple tenants. Furthermore, we highlight the future challenges and research directions regarding network softwarization and slicing using SDN and NFV in 5G networks.\cite{barakabitze_5g_2020} \par


Manufacturing has evolved over the course of centuries from the days of handmade goods to the adoption of water- and steam-powered machines, the invention of mass production, the introduction of electronic automation, and now beyond. Today, the benchmark for companies to keep up with, is Industry 4.0. Here, Manufacturing systems go beyond simple connection, to also communicate, analyse and use collected information to drive further intelligent actions. It represents an integration of IoT, analytics, additive manufacturing, robotics, artificial intelligence, advanced materials, and augmented reality. The paper looks at the evolution of the Industrial revolution and the technologies that have impacted their growth. The proposed features of 5G technologies are listed and described how these features impact the Industries of the future, leading to Industries 4.0. 5G promises to be a key enabler for Factories of the Future, providing unified communication platform needed to disrupt with new business models and to overcome the shortcomings of current communication technologies.\cite{rao_impact_2018} \par


The concept of “Smart Cities” is very important as it aims to uplift the living standards of the residents by greatly improving the City’s Infrastructure, Traffic management, Governance, Water and Waste management, Power management, Health systems, Safety and Security systems, Education systems etc. This paper describes the concept of Smart Cities and enumerates its various benefits. It describes various Services and Applications required to make a City Smart and the role of ICT technologies in their implementation. Further, the challenges in the current ICT systems are discussed in their role to Smart City implementation. The paper discusses the proposed features of 5G technologies and describes how 5G could be the best answer for successful, implementation of Smart Cities. It lists down a few Smart City Use Cases which are enabled by 5G. 5G will act as the backbone of IoT and pave the way for the development of Smart Cities.
\cite{rao_impact_2018-1} \par


The papers in this special section examine artificial intelligence (AI)-driven developments in 5G mobile communications for industrial automation applications from a Big Data perspective. With the recent advances in information and communication technologies, industrial automation is expanding at a rapid pace. This transition is characterized by “Industry 4.0”, the fourth revolution in the field of manufacturing. Industry 4.0, also called as “Industrial Internet of Things (IIoT)” or “Smart Factories”, is a reflection of new industrial revolution that is not only interconnected, but also communicate, analyze, and use the information to create a more holistic and better connected ecosystem for the industries.
\cite{garg_guest_2020} \par


The rise of Industry 4.0 is pushing more machine devices into the connection of the communication network. Internet of Things (IoT) emerges as an enabling technique to support automatic information transmission and the universal interconnection among massive machine devices. Unlike the human type communication (HTC) in the conventional Internet, IoT features machine type communication (HTC) with small data granularity and massive connections, which impose new challenges on the network resource allocation earlier designed for HTC communication. One of the challenging issues is how we can manage the network resource for the IoT service provisioning. As a promising network architecture for the “last-mile” access in 5G communication, Fiber-Wireless (FiWi) access network compromises the high bandwidth capacity of the optical access network and the flexibility of wireless access network. Especially, network virtualization as an emerging technique provides FiWi with the feasibility for the coordinated bandwidth allocation of wireless access network and optical access network. The evolution of FiWi access network should be not only oriented to the technological breakthrough in regular traffic, but also be supportive of the emerging IoT traffic. In this paper, we focus on the resource allocation problem in FiWi access network supporting IoT service. We first analyze the dynamics of regular traffic and propose the traffic prediction method based on Q-Learning. Then, we propose a virtual network embedding algorithm to map exactly the virtual networks of IoT traffic to the idle resource of the virtual networks of regular traffic without degrading the performance of regular traffic. Thus, the proposed algorithm can improve the resource utilization more effectively. The simulation results demonstrate that the proposed algorithm can achieve a higher acceptance ratio and lower migration ratio of IoT traffic.
\cite{liu_virtual_2019} \par

%Securing  the  communication  between  smart  industrialdevices
Wireless sensor networks (WSNs) have evolved to become an integral part of the contemporary Internet of Things (IoT) paradigm. The sensor node activities of both sensing phenomena in their immediate environments and reporting their findings to a centralized base station (BS) have remained a core platform to sustain heterogeneous service-centric applications. However, the adversarial threat to the sensors of the IoT paradigm remains significant. Denial of service (DoS) attacks, comprising a large volume of network packets, targeting a given sensor node(s) of the network, may cripple routine operations and cause catastrophic losses to emergency services. This paper presents an intelligent DoS detection framework comprising modules for data generation, feature ranking and generation, and training and testing. The proposed framework is experimentally tested under actual IoT attack scenarios, and the accuracy of the results is greater than that of traditional classification techniques.
\cite{baig_averaged_2020}\par

Blockchain – also known as distributed ledger – technology is set to revolutionise data and business process management and transactions. Blockchain adoption, pioneered initially as a financial technology (fintech) then as a supply chain technology (Underwood 2016), has expanded to public administration, transport, and logistics. Use cases in the former have been reported, but little is understood on its disruption in transport and logistics – including freight and passenger dimensions.

There is rising importance for a frictionless process where mobility of goods and services flow seamlessly between borders. There is a need for closer alignment between transport infrastructure including customs, airports, ports, rail and road. A digital infrastructure including clouds, intelligence management, payment systems, and pass-porting, to support these needs is paramount. This integration can enhance trade relations and transform the global supply chain. It can also transform how resources and capabilities in this environment can become more collaborative in the machine economy.

Industry, government or academic-led studies can provide novel insights to advance transformational impact in addressing challenge-led problems in public and private manufacturing and services. There is a need for research in a multi-modal transport and logistics environment, especially those incorporating legacy and future systems.

Within this context, there are also various global social and economic shifts occurring. Major globally impactful transitions such as One Belt-One Road led by China (Ferdinand 2016), increasing importance of airport resilience and operational efficiency (Rotondo 2019), Brexit – Global Britain (Tielmann and Schiereck 2017; Toly 2017), Shift2Rail (shift2rail.org), and other broad socio-economic transitions also relate to technological evolution of blockchains.

The transdisciplinarity of this issue is evident; multiple disciplines and a variety of stakeholders need to cooperate for taking full advantage of blockchain and related technology. Multiple methodologies for investigation are needed. Empirical research as well as new theoretical grounding, concepts, models and methods are likely necessary. Demonstration of blockchain adoption in related supply chain, manufacturing and service sectors for transport and logistics such as automotive, aviation, shipping, rail network, taxi-hailing service, forwarding, delivery service, travel require elaboration and synthesis.

This position paper aligned with the International Journal of Production Research Special Issue on Blockchain in Transport and Logistics aims to provide a foundation for the cutting-edge leading cases of the adoption of blockchain in transport and logistics, and chart the next wave of blockchain’s transformational role in transport and logistics. This position paper presents key concepts and methods informing the paradigms in blockchain for transport and logistics, and summarises various future directions and scenarios for blockchain transitions.
\cite{koh_blockchain_2020}\par



Following the great success of 2G and 3G mobile networks and the fast growth of 4G, the next generation mobile networks or 5th generation wireless systems (in short 5G) was proposed aiming to provide infinite networking capability to mobile users. Different from 4G, 5G is much more than increased maximum throughput. It aim to involve and benefit from many current technical advances including massive dense networks, interference and mobility management, Internet of Things (IoT), pervasive and social computing, mobile ad hoc networks (MANET), cognitive radio, World Wide Wireless Web (WWWW), cloud computing, IPv6, and so on. How 5G should and will be, what will be the keys for 5G? What is the perspective of 5G architecture and technologies? How to effectively apply and benefit from the above technologies and make them intelligently interoperate together? How can 5G stimulate our innovation for the next generation of mobile networks and services? Obviously, integrating all above existing advanced technologies and innovating new techniques for 5G bring extreme challenges on 5G networks and services in both research and development. This study has just initiated in both industry and academia, but with great fervor all over the world.
\cite{hu_editorial_2018}\par


The expanded deployment of smart objects in IoT applications is pushing existing IoT platform architectures and their security functionalities to their limits. Indeed, smart objects exhibit semi-autonomous behaviours, are not centrally controlled all the time and therefore need more dynamic approaches in protecting them against vulnerabilities and security incidents. In this paper, we introduce a novel framework for securing the latest generation of IoT applications that involve smart objects, while illustrating its application in securing an Ambient Assisted Living (AAL) system that comprises socially assistive robots.The framework{\textquoteright}s innovative aspects lie in the use of predictive analytics for anticipating the behaviour of smart objects, including abnormalities in their security behaviour. The importance of anticipating such abnormalities is validated, demonstrated and discussed in the context of the AAL application.
\cite{soldatos_securing_2020}\par



%Communication  Decision  support  in  smart  manufactur-ing:

The changing nature of manufacturing, in recent years, is evident in industry’s willingness to adopt network-connected intelligent machines in their factory development plans. A number of joint corporate/government initiatives also describe and encourage the adoption of Artificial Intelligence (AI) in the operation and management of production lines. Machine learning will have a significant role to play in the delivery of automated and intelligently supported maintenance decision-making systems. While e-maintenance practice provides aframework for internet-connected operation of maintenance practice the advent of IoT has changed the scale of internetworking and new architectures and tools are needed. While advances in sensors and sensor fusion techniques have been significant in recent years, the possibilities brought by IoT create new challenges in the scale of data and its analysis. The development of audit trail style practice for the collection of data and the provision of acomprehensive framework for its processing, analysis and use should be avaluable contribution in addressing the new data analytics challenges for maintenance created by internet connected devices. This paper proposes that further research should be conducted into audit trail collection of maintenance data, allowing future systems to enable ‘Human in the loop’ interactions.\cite{turner_intelligent_2019}\par

The future fifth-generation (5G) networks are expected to support a huge number of connected devices with various and multitude services having different quality of service (QoS) requirements. Communication in Industry 4.0 is one of the flagships and special applications of the 5G due to the specificity of the industrial environment as well as the variety of its services such as safety communication, robot's communications, and machine monitoring. In this context, we propose a new resource allocation for the future Industry 4.0 based on software-defined networking and network function virtualization technologies, machine learning tools and the slicing paradigm where each slice of the network is dedicated to a category of services having similar QoS requirement level. In this article, the proposed solution ensures the allocation of the resources to the slices depending on their requirements in terms of bandwidth, delay, and reliability. Toward this goal, our solution is performed in three main steps: first, Internet of Things (IoT) devices assignment to the slices step based on online Gaussian mixture model clustering algorithm, second, inter-slices resources reservations step based on mini-batch gradient descent, and third, intra-slices resources allocations based on the max-utility algorithm. We have performed extensive simulations in a realistic industrial scenario using NS3 simulator. Numerical results show the effectiveness of our proposed solution in terms of reducing packet error rate, energy consumption, and in terms of increasing the percentage of served devices in delay comparing to the traditional approaches.
\cite{messaoud_online_2020}\par

The role of digital technologies in service business transformation is under-investigated. This paper contributes to filling this gap by addressing how the Internet of things (IoT), cloud computing (CC) and predictive analytics (PA) facilitate service transformation in industrial companies. Through the Data–Information–Knowledge–Wisdom (DIKW) model, we discuss how the abovementioned technologies transform low-level entities such as data into information and knowledge to support the service transformation of manufacturers. We propose a set of digital capabilities, based on the extant literature and the findings from four case studies. Then, we discuss how these capabilities support the service transformation trajectories of manufacturers. We find that IoT is foundational to any service transformation, although it is mostly needed to become an availability provider. PA is essential for moving to the performance provider profile. Besides providing scalability in all profiles, CC is specifically used to implement an industrialiser strategy, therefore leading to standardised, repeatable and productised offerings.
\cite{ardolino_role_2018}\par

The term Tactile Internet broadly refers to a communication network that is capable of delivering real-time control, touch, and sensing/actuation information through sufficiently reliable, responsive, and intelligent connectivity. Envisioned to enable unprecedented applications, the Tactile Internet provides a promising opportunity to reshape industrial communication and transform the operation of many existing industrial systems. This paper investigates the role of Tactile Internet in current and future industrial systems and reviews the technological trends from legacy industrial networks to emerging industrial wireless networks, and beyond. To this end, this paper begins with an overview of the Tactile Internet. Complementing prior efforts, it presents a taxonomy of the key Tactile Internet applications. This paper covers the relevant background on the emergence of industrial communication. Then, it discusses the role of the Tactile Internet for various industrial systems and identifies the key use cases with respective connectivity requirements. This paper provides a technology landscape for the Tactile Internet to enable high-performance industrial wireless communication. Specifically, it provides insights into the recent Third Generation Partnership Project developments for enabling ultrareliable and low-latency communications over 5G mobile/cellular networks. It also examines the potential of the IEEE 802.11 and IEEE 802.15 standards for industrial control applications. Besides, it reviews the role of artificial intelligence and edge-computing platforms in overcoming the imperfections of wireless environments. Finally, this paper provides a roadmap for future, investigating the role of Tactile Internet in next generation industrial systems along with some directions and challenges for future research.
\cite{aijaz_tactile_2019}\par

Ambient assisted living provides an environment to aid regular activities (such as exercise, medical diagnosis etc.) for well being of users. In this direction, posture correcting mechanisms can be developed to have a real-time detection and correction system, which allow doctors and caregivers to monitor the patients’ health without worrying about potential falls and backaches. Most of the data related to patient health resides on the cloud environment to be accessed from anywhere by different users. However, the existing cloud computing infrastructure does not support a quick feedback for posture correction by the patients located geographically separated locations.However, with the advent of 5G networks, a new networking paradigm of Tactile Internet emerges having low latency communication for ubiquitously connecting heterogeneous devices at the edge of the network. Keeping focus on these issues, we propose, TILAA, a framework for Tactile Internet-based Ambient Assistance Living in fog environment in this paper. It provides a collaborative communication feedback to the patients and doctors with reduced delay. TILAA consists of a micro controller, sensing devices such as-accelerometer and gyroscopes, and a battery holder. The straps on the chest wearable consist of actuators, which send vibrations as a Tactile feedback to the doctors or to the hospitals for taking proactive measures in case of emergency. Performance evaluation of TILAA shows that it has superior performance for the back posture of all patients as compared to pre-existing expensive detection and posture schemes.
\cite{vora_tilaa_2019}\par


%Disruption in Wireless Communication Services :

The transformation of mobile networks towards fifth generation (5G) is considered an unprecedented revolution when compared to the previous generations, mainly because of the support required for three scenarios: ultra reliable and low latency; high throughput broadband; and massive machine type communication. In this context, the evolution from RAN to C-RAN is a significant contribution to advance the deployment of this new generation. C-RAN concepts bring opportunities like centralized processing, improved interference control, flexible fronthaul networks, and support for ultra-dense heterogeneous radio access networks. SDN emerges as a candidate technology for the development of programmable 5G networks, with centralized orchestration and control/data planes decoupling. In this article, we propose a systematic literature review to cover SDN application in the context of 5G communication and C-RAN. In combination with the concepts as mentioned earlier, the article evaluates coordination and interference management features provided by Coordinated Multi-point and Inter-cell Interference Coordination techniques, besides reviewing fronthaul transport tier capabilities offered by SDN for 5G networks. A careful literature analysis shows that there are no revisions with the same focus as that developed in this survey. As contributions, this article presents a novel taxonomy of SDN technology, enabling C-RAN, as well as trending directions and development opportunities for SDN and C-RAN-based 5G networks.\cite{zanferrari_morais_when_2020} \par

The Internet of Things (IoT) has become increasingly influential, particularly because of the significant new developments in the technologies of big data, cloud computing, 5G, and artificial intelligence. In this paper, we briefly explain how these new developments in the IoT may create a new electronic commerce landscape and opportunities associated with it; these developments pose interesting questions for future research.\cite{zhang_2020_2020} \par

Production Research is foundational for advancing theories, methods, technologies and practices in manufacturing industries, production systems and related service industries. Over the last five decades, tremendous scientific and technical progresses have been made in all areas of production of goods and services, ranging from the birth of Computer-Aided tools (CAx, where x stands for Design, Manufacturing, Process Planning or Engineering), Computer Numerically Controlled (CNC) machines and industrial robotics in the 60s, then to Flexible Manufacturing Systems (FMSs), Automated Guided-Vehicles (AGVs) and concept of unmanned factories in the 70s, to Computer-Integrated Manufacturing (CIM), quality management, value chains and lean management in the 80s, to mass customisation, distributed warehousing and networked organisations governed by integrated Enterprise Resource Planning (ERP) packages in the 90s, then to service-orientation (or ‘servitization’), global supply chains and interoperable and knowledge-based systems in the 2000s and, finally, to emerging smart, sensing and sustainable production systems today culminating with the concept of smart factories and Industry 4.0 since 2011, and the emerging cyber physical production. \cite{vernadat_information_2018} \par


%Industrial Innovation and Infrastructure
As  the  trust  in  the  automated  decision  making  by  smartindustrial  machines  using  artificial  intelligence  are  getting  aserious  concern,  the  demand  for  trust  worthy  machines  aregaining  importance.  Explainable  artificial  intelligence  (XAI)has  emerged  as  a  transparent  mechanism  for  predicting  therequirements in automated industry with complete exploitationof Industry 4.0 [196] \cite{rehse2019towards}

Internet of Things (IoT) has gain the importance with the growing applications in the fields of ubiquitous and context-aware computing. In IoT, anything can be a portion of it, whether it is unintelligent objects or sensor nodes; thus extremely different kinds of services can be developed. In this regard, data storage, resource management, service creation and discovery, and resource and power management would facilitate advanced mechanism and much better infrastructure. Cloud computing and fog computing play an important role when the quantity of data and information IoT are critical. Thus, it would not be potential for standalone strength forced IoT to handle. Cloud of things is an integration of IoT with cloud computing or fog computing which can aid to realize the objectives of evolving IoT and future Internet. Fog computing is an expansion to the notion of cloud computing to the network brim, making it suitable for IoT and other implementations that need real-time and fundamental interactions. Regardless of many virtually and services unlimited resources presented by cloud-like intelligent building monitoring and others, it yet countenances various difficulties when interfering many smart things in human's life. Mobility, response time, and location consciousness are the most prominent problems. Fog and mobile edge computing have been established, to get rid of these difficulties of cloud computing. In this article, we suggest a novel framework based on computer propped diagnosis and IoT to detect and observe type-2 diabetes patients. The recommended healthcare system aims to obtain a better accuracy of diagnosis with mysterious data. The overall experimental results indicate the validity and robustness of our proposed algorithms.
\cite{abdel-basset_novel_2019}\par

The role of the Industrial Internet of Things (IIoT) in critical infrastructure sectors, such as power, chemistry, and manufacturing, will be increasingly important as we move toward Industry 5.0. For example, IIoT devices are deployed in factories to help the manufacturing companies (e.g., automotive) gain in-depth insight into the various states of production, and thus improving production efficiency and achieving cost reductions. However, malicious code may compromise IIoT devices if either the devices are exposed to outside or unexposed inner devices are updated unauthentically. Due to their limited resources and features, it is challenging to implement strong security solutions for such embedded devices. In this article, we propose a blockchainbased software status monitoring system, called BoSMoS. The
system is designed to monitor the software status of IIoT devices to detect and respond to identified malicious behaviors (e.g., intrusions). BoSMoS takes a snapshot of the statue of monitored software and monitors its file system calls. In order to ensure the software integrity information, we use blockchain as the distributed ledger to store a snapshot of software status. The blockchain network of BoSMoS can employ different consensus algorithms. We also evaluate the performance of BoSMoS, in terms of exception response delay, resistance performance to various intrusions, and scalability. The experimental results justify that BoSMoS is practical and sound. In addition, the evaluation of scalability and security demonstrates that the system can carry deployment of large-scale IIoT devices and can guarantee authenticated software updating, as well as detect unauthorized software status.
\cite{he_bosmos_2020}\par

The significant advancement in the fields of electronics and computer science has produced innovation in devices and systems. For example, the miniaturisation of electronic components and devices combined with the evolution of wireless distributed networks have significantly enabled mobility and the connectivity of devices. Also, advances in sensor technologies have allowed ubiquitous objects to measure performance and transmit information regarding their functional state and their operating environment in a more reliable and low-cost way. These technologies enabled the development of mobile devices and wearable electronics. In addition, Web 2.0, fast-speed computing and efficient data storage have facilitated the emergence of new generation of data analytics and machine learning. Taken together, these plethora of new advanced technologies offer numerous possibilities and pitfalls for users. It is argued that they will change our world and whatever we do at work, home, leisure and even during times of crisis (Elbanna et al. 2019; Hughes et al. 2019; Ismagilova et al. 2019a, b; Kim et al. 2016; Papagiannidis and Marikyan 2019; Rana et al. 2019; Bunker et al. 2019b; Stieglitz et al. 2018). One of the changes receiving currency is the capability of these technologies to be ‘smart’ and to make us ‘smart’. While the the term ‘smart’ is used vaguely by management and in the corridors of policy makers, computer scientists typically associate it with the use of the internet, connected devices, embedded sensors and machine learning. In this special issue, we widen the definition of ‘smart’ from a narrow technically oriented view to a wider transformatory sociotechnical view that puts use, impact and outcomes at the heart of achieving smartness in working, living and organising. Smart here is defined as ‘the intelligent and rational use of resources to work, organise and live efficiently and effectively, healthily and happily, to the benefits of individuals, society, humankind and planet earth’.
\cite{elbanna_search_2020}\par

Industry 4.0 is taking human-robot collaboration at the center of the production environment. Collaborative robots enhance productivity and flexibility while reducing human’s fatigue and the risk of injuries, exploiting advanced control methodologies. However, there is a lack of real-time model-based controllers accounting for the complex human-robot interaction dynamics. With this aim, this paper proposes a Model-Based Reinforcement Learning (MBRL) variable impedance controller to assist human operators in collaborative tasks. More in details, an ensemble of Artificial Neural Networks (ANNs) is used to learn a human-robot interaction dynamic model, capturing uncertainties. Such a learned model is kept updated during collaborative tasks execution. In addition, the learned model is used by a Model Predictive Controller (MPC) with Cross-Entropy Method (CEM). The aim of the MPC+CEM is to online optimize the stiffness and damping impedance control parameters minimizing the human effort (i.e, minimizing the human-robot interaction forces). The proposed approach has been validated through an experimental procedure. A lifting task has been considered as the reference validation application (weight of the manipulated part: 10 kg unknown to the robot controller). A KUKA LBR iiwa 14 R820 has been used as a test platform. Qualitative performance (i.e, questionnaire on perceived collaboration) have been evaluated. Achieved results have been compared with previous developed offline model-free optimized controllers and with the robot manual guidance controller. The proposed MBRL variable impedance controller shows improved human-robot collaboration. The proposed controller is capable to actively assist the human in the target task, compensating for the unknown part weight. The human-robot interaction dynamic model has been trained with a few initial experiments (30 initial experiments). In addition, the possibility to keep the learning of the human-robot interaction dynamics active allows accounting for the adaptation of human motor system.
\cite{roveda_model-based_2020}\par

Technological advances have made possible industrial and commercial applications of artificial intelligence, virtual reality and highly integrated manufacturing systems. It has also freed business activity from a focus on place, as both work activities and markets have been able to harness information and communication technologies in order to operate remotely. As a result, researchers have highlighted a phenomenon of ‘smart’ working. Some have pointed to a fourth Industrial Revolution (Industry 4.0) in which ‘smart’ factories use robotics to achieve high performance. There is now a suggestion of progress towards Industry 5.0, in which technological and social systems work in harmony to deliver personalised mass customization of products and services. This paper examines these developments from the perspective of unique, individual understandings of work roles and sustainability, posing the questions ‘Smart’ from whose point of view? Do smart systems promote sustainable organizations? How should design of smart systems be approached? It suggests that contemporary socio-technical systems approaches to organizational analysis are the best way to support harnessing of smart technologies in organizations.
\cite{bednar_socio-technical_2019}\par

My objective is to create an intuitive computer for laypeople who want to go beyond ready-made apps and create programs to control their electronic environment. I submit Loke, a new kind of computer that is a universe of objects and nothing but objects. I call it an object computer. Loke is implemented in Squeak, a variant of Smalltalk, and is an extensible, conceptual model for execution, inspection, and exploration. It was first used to demonstrate how Ellen, a novice, programs a smart alarm clock through a GUI adapted to her competence, needs, and preferences. Informal demonstrations indicated that laypeople immediately grasp the idea of communicating objects that represent real things in their environment. They also wanted to use it for their own purposes. They were creative in identifying personal opportunities for Loke and in sketching out their implementations. Interestingly, expert programmers who attended the demonstration did not see the point of Loke. I have completed the programming of Loke qua conceptual model. The model underpins its potential security and privacy and sustains its object and message models. The Loke qua programming environment is still in its infancy, and its inherent security and privacy properties are still not realized in practice. A future Loke device will be accessible from anywhere and embedded in its own hardware to achieve them. The Loke IDE rests on Data–Context–Interaction (DCI), a new programming paradigm that leads to readable code with a clear architecture. 
\cite{reenskaug_personal_2019}\par



% Sustainability in Industrial Revolution

Robotics for domestic services

Manufacturing industry profoundly impact economic and societal progress. As being a commonly accepted term for research centers and universities, the Industry 4.0 initiative has received a splendid attention of the business and research community. Although the idea is not new and was on the agenda of academic research in many years with different perceptions, the term “Industry 4.0” is just launched and well accepted to some extend not only in academic life but also in the industrial society as well. While academic research focuses on understanding and defining the concept and trying to develop related systems, business models and respective methodologies, industry, on the other hand, focuses its attention on the change of industrial machine suits and intelligent products as well as potential customers on this progress. It is therefore important for the companies to primarily understand the features and content of the Industry 4.0 for potential transformation from machine dominant manufacturing to digital manufacturing. In order to achieve a successful transformation, they should clearly review their positions and respective potentials against basic requirements set forward for Industry 4.0 standard. This will allow them to generate a well-defined road map. There has been several approaches and discussions going on along this line, a several road maps are already proposed. Some of those are reviewed in this paper. However, the literature clearly indicates the lack of respective assessment methodologies. Since the implementation and applications of related theorems and definitions outlined for the 4th industrial revolution is not mature enough for most of the reel life implementations, a systematic approach
\cite{oztemel_literature_2020}\par

In this paper are investigated the re-engineering approaches for the optimization of pasta production processes. A preliminary study of technologies and information systems architectures to be applied to the entire pasta supply chain has been carried out. In the first part of the paper is presented an overview concerning Industry 4.0 enabling technologies, besides, in the second part are discussed the engineered processes improving production quality. Concerning simulation process, is designed by means of modelling workflows the wheat storage process, by simulating the automatism of silos controlled and managed by volume sensors. Finally, following Industry 5.0 facilities have been applied image vision and artificial intelligence methodologies suitable for auto-adaptive quality check of pasta. The paper discusses different models about production processes, efficiency, risks, costs and benefits.
\cite{massaro_re-engineering_2020}\par

Globally cities are becoming experimental sites for new forms of robotic and automation technologies applied across a wide variety of sectors in multiple areas of economic and social life. As these innovations leave the laboratory and factory, this paper analyzes how robotics and automation systems are being layered upon existing urban digital networks, extending the capabilities and capacities of human agency and infrastructure networks, and reshaping the city and citizen’s everyday experiences. To date, most work in this field has been speculative and isolated in nature. We set out a research agenda that goes beyond analysis of discrete applications and effects, to investigate how robotics and automation connect across urban domains and the implications for differential urban geographies, the selective enhancement of individuals and collective management of infrastructures, the socio-spatial sorting of cities and the potential for responsible urban innovation.
\cite{macrorie_robotics_2019}\par


The adoption of emerging technological trends and applications of the Internet of Things (IoT) in the industrial systems is leading towards the development of Industrial IoT (IIoT). IIoT serves as a new vision of IoT in the industrial sector by automating smart objects for sensing, collecting, processing and communicating the real-time events in industrial systems. The major objective of IIoT is to achieve high operational efficiency, increased productivity, and better management of industrial assets and processes through product customization, intelligent monitoring applications for production floor shops and machine health, and predictive and preventive maintenance of industrial equipment. In this paper, we present a new and clear definition of IIoT, which can help the readers to understand the concept of IIoT. We have described the state-of-the-art research efforts in IIoT. Finally, we have highlighted the enabling technologies for IIoT and recent challenges faced by IIoT.
\cite{khan2020industrial}\par

In recent years, the bioeconomy has established itself worldwide as a mainstay for achieving a sustainable economy. The targeted use of biological resources for industrial purposes can help to successfully reconcile ecology and economy in the long term. Like digitalization, biologization as the guiding principle of the bioeconomy has the potential to effect a fundamental change in industry. This change must be driven and supported by a committed research and innovation policy. The German Federal Government was one of the first governments worldwide to put the bioeconomy on its research policy agenda when it adopted the “National Research Strategy BioEconomy 2030” in 2010. The respective national policy strategy was published two years later. Since then we have been successfully implementing measures to establish the bioeconomy. Our research programme is currently being developed further. Our aim is to strengthen the biobased transformation process towards a sustainable economy and to attach special importance to innovative technologies. Furthermore, bioeconomy research policy will have to be aimed more strongly towards achieving international goals such as the Sustainable Development Goals (SDGs) and to showing what contribution the bioeconomy can make in this context. The success of the bioeconomy requires a societal discourse on how our society can reconcile economic growth and sustainability in future. This requires the adaptation and continued development of national agendas and initiatives as well as efficient international cooperation.
\cite{schutte_what_2018}\par



% ------------------------------------------------------------------------------------------
\begin{table*}
%\centering
\scriptsize
\caption{Summary of Existing Surveys related to Artificial Intelligence and Industry 4.0} \textcolor{blue}{WE NEED TO REFINE THE TABLE please add data-related challenges, explainability, and adversarial ML. this will help to differentiate it from the existing work.} % can we add another column to show the year of the publication of each paper?}}}
\label{tab:survey}
\begin{tabular}{|>{\arraybackslash}p{2cm}|>{\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.7cm}|>{\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.7cm}|>{\centering\arraybackslash}p{0.7cm}|>{\arraybackslash}p{5.5cm}|}
 \hline
\textbf{Refs. (Author)}
& \textbf{Year}
& \textbf{\tiny AI 4.0 \newline Review} 
& \textbf{\tiny Smart \newline Manufacturing}
& \textbf{\tiny IIoT \newline Review}
& \textbf{\tiny Robotics \newline Review}
& \textbf{\tiny Big Data \newline Analytics}
& \textbf{\tiny Security \& Privacy}
& \textbf{\tiny Regulatory \newline Issues}
& \textbf{\tiny Overview}
 \\ \hline \hline
 
% ########################################################################\

Aceto et al.~\cite{aceto_survey_2019} & 2019 & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \xmark{} & Analysis on the integration of key technology enablers for Industry 4.0 \\ \hline

% ########################################################################

Lu et al.~\cite{lu2017industry} & 2017 & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & Examines the critical issues in interoperability and proposed a conceptual framework for Industry 4.0
\\ \hline

% ########################################################################

Zhong et al.~\cite{zhong2017intelligent}  & 2017 &\checkmark{} & \checkmark{} & \checkmark{} & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & Strategic plans for intelligent manufacturing are highlighted and analyzed \\\hline

% ########################################################################

Oztemel et al.~\cite{oztemel2020literature} & 2020 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & With six design principles the conceptual framework of Industry 4.0 is analyzed \\ \hline

% ########################################################################

Xu et al.~\cite{xu2019big} & 2019 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & Surveys about research direction on complete autonomous operations in Industry 4.0 \\ \hline

% ########################################################################

Kamble et al.~\cite{kamble2018sustainable} & 2018 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & Industry 4.0 framework is proposed for sustainable smart manufacturing \\ \hline

% ########################################################################

%Alcacer et al.~\cite{alcacer2019scanning} & 2019 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & Digital platforms for smart manufacturing are discussed with the support of enabling technologies \\ \hline

% ########################################################################

%Liao et al.~\cite{liao2017past} & 2017 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Hardware and software standards for Industry 4.0 are reviewed based on data analysis \\ \hline

% ########################################################################

%Bodkhe et al.~\cite{bodkhe2020blockchain} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & ?? & Using appropriate reference architectures, blockchain based security solutions for Industry 4.0 applications are analyzed \\ \hline

% ########################################################################
Pereira et al.~\cite{pereira2017review} & 2017 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & Drives to develop new business models for Industry 4.0 considering various technological implications \\ \hline

% ########################################################################

%Manavalan et al.~\cite{manavalan2019review} & 2019 & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & Transformation readiness towards Industry 4.0 are assessed from five different perspectives \\ \hline

% ########################################################################

%Dallasega et al.~\cite{dallasega2018industry} & 2018 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & Using practical industrial case studies frameworks for Industry 4.0 are discussed \\ \hline

% ########################################################################

Mittal et al.~\cite{mittal2018critical} & 2018 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & Impact and contribution of smart manufacturing in medium sized enterprises are summarized with smart manufacturing models \\ \hline

% ########################################################################

Alladi et al.~\cite{alladi2019blockchain} & 2019 & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & Challenges in blockchain implementation for Industry 4.0 in conjugation with IIoT are addressed with the application domains \\ \hline

% ########################################################################

Kerin et al.~\cite{kerin2019review} & 2019 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & Key observations from 29 research topics related to Industry 4.0 are summarized \\ \hline

% ########################################################################

Osterrieder et al.~\cite{osterrieder2020smart} & 2020 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Research model for smart manufacturing is put forward for future research in this domain \\ \hline

% ########################################################################

%Fernandez et al.~\cite{fernandez2018review} & 2018 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Smart labeling in industries are addressed from human-centric perspective \\ \hline

% ########################################################################

%Da et al.~\cite{da2019technology} & 2019 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & Stages of supply chain are addressed with technology transfer support towards Industry 4.0 \\ \hline

% ########################################################################

Davies et al.~\cite{davies2017review} & 2017 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Importance of soci-technical requirements for lean manufacturing are reviewed \\ \hline

% ########################################################################

Khan et al.~\cite{khan2016survey} & 2016 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & New technology and tools are introduced to support the growth of Industry 4.0 \\ \hline

% ########################################################################

Trappey et al.~\cite{trappey2017review} & 2017 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Impact of IoT standards for enhancing the productivity in smart manufacturing are reviewed with case studies \\ \hline

% ########################################################################

Yli et al.~\cite{yli2019adapting} & 2019 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & Communication and networking standards for agile manufacturing are summarized \\ \hline

% ########################################################################

Sanchez et al.~\cite{sanchez2020industry} & 2020 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & Collaboration, organization and system integration features for Industry 4.0 are discussed \\ \hline

% ########################################################################

Preuveneers et al.~\cite{preuveneers2017intelligent} & 2017 & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & Recent developments and challenges in intelligent manufacturing are addressed \\ \hline

% ########################################################################

%Klingenberg et al.~\cite{klingenberg2019industry} & 2019 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & Framework for handling industrial data and providing effective value for them are addressed \\ \hline

% ########################################################################

%Beier et al.~\cite{beier2020industry} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Sustainability concerns in Industry 4.0 are reviewed from sociotechnical perspective \\ \hline

% ########################################################################

Kim et al.~\cite{kim2017review} & 2017 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & Imparting data security in CPS systems for Industries are reviewed \\ \hline

% ########################################################################

Sony et al.~\cite{sony2020critical} & 2020 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Critical factors are addressed for sustainable implementation of Industry 4.0 \\ \hline

% ########################################################################

Li et al.~\cite{li2017review} & 2017 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Design challenges in wireless networking for smart industries are discussed \\ \hline

% ########################################################################

Souza et al.~\cite{souza2020survey} & 2020 & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & From the context of Industry 4.0, how strategic decisions affect the reliability of products are summarized \\ \hline

% ########################################################################

Leng et al.~\cite{leng2020blockchain} & 2020 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & Successful empowerment of blockchain technology amidst the challenges in industries are addressed \\ \hline

% ########################################################################

%Liu et al.~\cite{liu2018cps} & 2018 & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & \xmark{} & Robotic systems involved in warehouse management with appropriate CPS are surveyed \\ \hline

% ########################################################################

Horst et al.~\cite{horst2018additive} & 2018 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & Integration of IIoT for 3D printing providing towards smart manufacturing prospects are discussed \\ \hline

% ########################################################################

Nunez et al.~\cite{nunez2020information} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Impact of digital technology supporting the policymakers for successful implementation of modern trends in industries are reviewed \\ \hline

% ########################################################################

Calabres et al.~\cite{calabrese2020evolutions} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Evolution and revolution aspects of Industry 4.0 are addressed for foreseeing the business prospects \\ \hline

% ########################################################################

Angelopoulos et al.~\cite{angelopoulos2020tackling} & 2020 & \checkmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & Machine learning based closed loop operation of human and machine are analyzed for using IIoT \\ \hline

% ########################################################################

Nguyen et al.~\cite{nguyen2020systematic} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & Handling of Big data effectively in oil \& gas industries are addressed with appropriate security measures \\ \hline

% ########################################################################

Prinsloo et al.~\cite{prinsloo2019review} & 2019 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & Security risks and their countermeasures are conceptualized for Industry 4.0 \\ \hline

% ########################################################################

Hernandez et al.~\cite{hernandez2020systematic} & 2020 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & Usage of modern tools for smart manufacturing are addressed using bibliometric analysis \\ \hline

% ########################################################################
ur Rehman et al.~\cite{ur_rehman_role_2019} & 2019 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & Case studies on IIoT and usage of big data analytics frameworks were explored. \\ \hline

% ########################################################################

Kumar et al.~\cite{kumar2020adversarial} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & Security enforcement using adversarial ML in smart industries are enumerated.  \\ \hline

% ########################################################################

Guidotti et al.~\cite{guidotti2018survey} & 2018 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & Provides explainable methods that could be used across multiple industries \\ \hline

% ########################################################################
Our Survey & 2021 & \checkmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \checkmark{} & Focuses the integration of AI with Smart manufacturing, IIoT, Big data, Security and regulatory standards \\ \hline

% ########################################################################

\end{tabular}
%\caption{Comparative analysis of our survey with the existing survey literature pool}
%\label{table:comparison}
\end{table*}











% ########################################################################\

Aceto et al.~\cite{aceto_survey_2019} & 2019 & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \xmark{} &  \xmark{}  &   & Analysis on the integration of key technology enablers for Industry 4.0 \\ \hline
A Survey on Information and Communication Technologies for Industry 4.0: State-of-the-Art, Taxonomies, Perspectives, and Challenges
% ########################################################################

Lu et al.~\cite{lu2017industry} & 2017 & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & \xmark{} & \xmark{} &  & Examines the critical issues in interoperability and proposed a conceptual framework for Industry 4.0
\\ \hline

Industry 4.0: A survey on technologies, applications and open research issues
% ########################################################################

Zhong et al.~\cite{zhong2017intelligent}  & 2017 &\checkmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \checkmark{} & & & &  Strategic plans for intelligent manufacturing are highlighted and analyzed \\\hline
Intelligent manufacturing in the context of industry 4.0: a review
% ########################################################################

Oztemel et al.~\cite{oztemel2020literature} & 2020 & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & \xmark{} & & & & With six design principles the conceptual framework of Industry 4.0 is analyzed \\ \hline
Literature review of Industry 4.0 and related technologie
% ########################################################################

Xu et al.~\cite{xu2019big} & 2019 & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & & & & Surveys about research direction on complete autonomous operations in Industry 4.0 \\ \hline
Big data for cyber physical systems in industry 4.0: a survey
% ########################################################################

Kamble et al.~\cite{kamble2018sustainable} & 2018 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & & & & Industry 4.0 framework is proposed for sustainable smart manufacturing \\ \hline
Sustainable Industry 4.0 framework: A systematic literature review identifying the current trends and future perspectives
% ########################################################################

Pereira et al.~\cite{pereira2017review} & 2017 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \checkmark{} & & & & Drives to develop new business models for Industry 4.0 considering various technological implications \\ \hline
A review of the meanings and the implications of the Industry 4.0 concept
% ########################################################################

Mittal et al.~\cite{mittal2018critical} & 2018 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & & & & Impact and contribution of smart manufacturing in medium sized enterprises are summarized with smart manufacturing models \\ \hline
A critical review of smart manufacturing \& Industry 4.0 maturity models: Implications for small and medium-sized enterprises (SMEs)
% ########################################################################

Alladi et al.~\cite{alladi2019blockchain} & 2019 & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & & & & Challenges in blockchain implementation for Industry 4.0 in conjugation with IIoT are addressed with the application domains \\ \hline
Blockchain applications for industry 4.0 and industrial IoT: A review
% ########################################################################

Kerin et al.~\cite{kerin2019review} & 2019 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \checkmark{} & & & & Key observations from 29 research topics related to Industry 4.0 are summarized \\ \hline
A review of emerging industry 4.0 technologies in remanufacturing
% ########################################################################

Osterrieder et al.~\cite{osterrieder2020smart} & 2020 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & & & & Research model for smart manufacturing is put forward for future research in this domain \\ \hline
The smart factory as a key construct of industry 4.0: A systematic literature review
% ########################################################################

Davies et al.~\cite{davies2017review} & 2017 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & & & & Importance of soci-technical requirements for lean manufacturing are reviewed \\ \hline
Review of socio-technical considerations to ensure successful implementation of Industry 4.0
% ########################################################################

Khan et al.~\cite{khan2016survey} & 2016 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & & & & New technology and tools are introduced to support the growth of Industry 4.0 \\ \hline
A survey of current challenges in manufacturing industry and preparation for industry 4.0
% ########################################################################

Trappey et al.~\cite{trappey2017review} & 2017 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & & & & Impact of IoT standards for enhancing the productivity in smart manufacturing are reviewed with case studies \\ \hline
A review of essential standards and patent landscapes for the Internet of Things: A key enabler for Industry 4.0
% ########################################################################

Yli et al.~\cite{yli2019adapting} & 2019 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \checkmark{} & & & & Communication and networking standards for agile manufacturing are summarized \\ \hline
Adapting an agile manufacturing concept to the reference architecture model industry 4.0: A survey and case study
% ########################################################################

Sanchez et al.~\cite{sanchez2020industry} & 2020 & \xmark{} & \checkmark{} & \checkmark{} & \xmark{} & \xmark{} & & & & Collaboration, organization and system integration features for Industry 4.0 are discussed \\ \hline
Industry 4.0: survey from a system integration perspective
% ########################################################################

Preuveneers et al.~\cite{preuveneers2017intelligent} & 2017 & \checkmark{} & \checkmark{} & \xmark{} & \checkmark{} & \checkmark{} & & & & Recent developments and challenges in intelligent manufacturing are addressed \\ \hline
The intelligent industry of the future: A survey on emerging trends, research challenges and opportunities in Industry 4.0
% ########################################################################

Kim et al.~\cite{kim2017review} & 2017 & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & & & & Imparting data security in CPS systems for Industries are reviewed \\ \hline
A review of cyber-physical system research relevant to the emerging IT trends: industry 4.0, IoT, big data, and cloud computing
% ########################################################################

Sony et al.~\cite{sony2020critical} & 2020 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & & & & Critical factors are addressed for sustainable implementation of Industry 4.0 \\ \hline
Critical factors for the successful implementation of Industry 4.0: a review and future research direction
% ########################################################################

Li et al.~\cite{li2017review} & 2017 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \xmark{} & & & & Design challenges in wireless networking for smart industries are discussed \\ \hline
A review of industrial wireless networks in the context of industry 4.0
% ########################################################################

Souza et al.~\cite{souza2020survey} & 2020 & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & & & & From the context of Industry 4.0, how strategic decisions affect the reliability of products are summarized \\ \hline
A survey on decision-making based on system reliability in the context of Industry 4.0
% ########################################################################

Leng et al.~\cite{leng2020blockchain} & 2020 & \xmark{} & \checkmark{} & \xmark{} & \xmark{} & \checkmark{} & & & & Successful empowerment of blockchain technology amidst the challenges in industries are addressed \\ \hline
Blockchain-empowered sustainable manufacturing and product lifecycle management in industry 4.0: A survey
% ########################################################################

Nunez et al.~\cite{nunez2020information} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & & & & Impact of digital technology supporting the policymakers for successful implementation of modern trends in industries are reviewed \\ \hline
Information and digital technologies of Industry 4.0 and Lean supply chain management: a systematic literature review
% ########################################################################

Calabres et al.~\cite{calabrese2020evolutions} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \xmark{} & & & & Evolution and revolution aspects of Industry 4.0 are addressed for foreseeing the business prospects \\ \hline
‘Evolutions’ and ‘revolutions’ in manufacturers’ implementation of industry 4.0: a literature review, a multiple case study, and a conceptual framework
% ########################################################################

Angelopoulos et al.~\cite{angelopoulos2020tackling} & 2020 & \checkmark{} & \xmark{} & \checkmark{} & \xmark{} & \checkmark{} & & & & Machine learning based closed loop operation of human and machine are analyzed for using IIoT \\ \hline
Tackling Faults in the Industry 4.0 Era—A Survey of Machine-Learning Solutions and Key Aspects
% ########################################################################

Nguyen et al.~\cite{nguyen2020systematic} & 2020 & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \checkmark{} & & & & Handling of Big data effectively in oil \& gas industries are addressed with appropriate security measures \\ \hline
A Systematic Review of Big Data Analytics for Oil and Gas Industry 4.0
% ########################################################################

ur Rehman et al.~\cite{ur_rehman_role_2019} & 2019 & \xmark{} & \checkmark{} & \checkmark{} & \checkmark{} & \xmark{} & & & & Case studies on IIoT and usage of big data analytics frameworks were explored. \\ \hline
The role of big data analytics in industrial {Internet} of {Things}
% ########################################################################

Kumar et al.~\cite{kumar2020adversarial} & 2020 & \xmark{} & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & & & & Security enforcement using adversarial ML in smart industries are enumerated.  \\ \hline
Adversarial Machine Learning--Industry Perspectives
% ########################################################################

Guidotti et al.~\cite{guidotti2018survey} & 2018 & \xmark{} & \xmark{} & \xmark{} & \checkmark{} & \xmark{} & & & & Provides explainable methods that could be used across multiple industries \\ \hline
A survey of methods for explaining black box models












==> IIOT_Data_handling.tex <==
\subsection{IIoT data handling and its trustworthiness in Industry 4.0}

In this subsection, we provide a detailed analysis of key challenges to IIoTs with potential solutions proposed in the literature.

\subsubsection{Digitization and Social Trends in Modern Industries}
Expectations of consumer segments are far beyond the current digital transformation. They need to monitor, operate, and control appliances without making much efforts. The evolution of IIoT has made a paradigm shift to meet expectations through smart industries and appliances. Smart devices can communicate effectively in the industrial environment with modern wireless communication technologies employed in IIoT enabled machines\cite{khan2020industrial}. IIoT being a subset of IoT are supported with numerous enabling technologies for the disruptive evolution of digitization in smart industries\cite{younan_challenges_2020}. Sustainable technologies for Industry 4.0\cite{ghobakhloo_industry_2020}, Socio-technical view of modern industries\cite{beier_industry_2020}, state of art tools for smart machines\cite{xu_industry_2018} are summarized by many researchers and compiled the significance of IIoT towards social trends in the manufacturing sector. %Fig. \ref{fig:IIoTAppl} shows the most common applications of IIoT, from the perspective of industry 4.0 implementation in smart industries. \par

Few researchers summarized the case studies of using IIoT in modern industries\cite{lu_oil_2019} with the potential requirement and challenges involved\cite{silva_implementation_2020} and new advancements of Industry 4.0\cite{hervas-oliver_place-based_2019} driving the paradigm shift of industrial manufacturing processes. Digitization of industries also invokes the demand for Cyber-Physical  System integration with IIoT\cite{kipper_scopus_2020} and improved cognitive ability in solving challenging socio-economic smart industrial environments\cite{zolotova_smart_2020}. \par

Adopting Industry 4.0 requires both vertical and horizontal data integration across various business segments. Vertical digitization includes procurement, product design, manufacturing, supply chain,  product life cycle management, logistics, operations, and quality of service; all integrated for seamless flow of data. Horizontal digitization includes data integration with suppliers, customers, and key partners. Achieving integration requires upgrading or replacing equipment, networks, and processes until a seamless digital ecosystem is established. \par   

%------------------------------------------------------------------------------
\subsubsection{IIoT Data Handling in Smart Manufacturing}
It is not enough to only have the digital systems completely integrated into the modern manufacturing sectors, concrete data analytical services also need to be established to turn the information generated by IIoT systems, sensors, and smart machines into actionable insights that can return on investments in the manufacturing process. Thus, sustainable smart manufacturing can be used for smooth life cycle management of the products manufactured in association with the IIoT data, Big Data analytics and ubiquitous servitization as proposed in\cite{ren_comprehensive_2019}. In the smart manufacturing eco-systems, throughput bottlenecks are one of the most common issues that may occur in the production line that generate data from machines in larger volumes. The authors in\cite{subramaniyan_data-driven_2018} implemented an auto-regressive integrated moving average method for predicting the machine behaviors in the active periods with the data acquired using the bottleneck prediction algorithm. Here, the data are channelized and handled effectively for overcoming the bottleneck issues and improves the throughput for enabling production tasks in a smooth way.\par

IIoT data collected from smart machines enabled with sensors in smart factories are also used for performing condition-based maintenance\cite{lin_concept_2019}. Specifically, three-stage condition-based maintenance is employed using an ensemble learning algorithm with the first stage involved in training the ensemble, the second stage detects the imbalance IIoT data and the final stage is involved in creating new ensembles. Experimental analysis on the condition-based maintenance provides high accuracy with better detection of all the drifts in the data. \par

Moreover, on one hand, the IIoT data collected by sensors in smart factories can efficiently be communicated to intelligent frameworks for translation and further analysis. The authors in\cite{peres_idarts_2018} aim to implement an Intelligent Data Analysis and Real-Time Supervision framework for the translation of IIoT data from the machines in smart industries. However, its integration with cyber-physical systems drives positive impact and provides prospective business advantage. Moreover, this framework also enables distribution acquisitions of data from IIoT devices thereby providing predictive maintenance with better quality control of the manufactured products. \par

On another hand, text mining on the IIoT data collected is another stream of the business prospect that governs Industry 4.0. The text mining data are used for suggesting better operations, technological solutions, improved work skills of the operators, and improved business opportunities\cite{galati_industry_2019}. Ensuring privacy in data mining is one of the key enablers for protecting massive sets of IIoT data from the machines in smart industries. Such large data sets are effectively managed with the minimized transfer of data across nodes using MapReduce frameworks\cite{keshk_privacy-preserving_2018}. This implies that the IIoT data could enhance manufacturing processes in smart industries in association with proper handling and analytics on the industrial data. \par 

%------------------------------------------------------------------------------
%\subsubsection{5G and Wireless Communication Services for IIoT }

%AI, IIoT, and 5G communication services are integrated to build smart industries with a well-connected ecosystem\cite{garg_guest_2020}. Seamless connectivity of 5G enabled Industry 4.0 demands the best vertical handover in a smart production environment and different application scenarios. Priya et al.\cite{priya_5gaunets_2019} addressed these issues under four application scenarios that employ 5G communication service. Those services are tested for effective vertical handover with hybrid models used in Bitpipe, Tactile Internet, IIoT, and regional areas with Internet access, and better performance are observed. \par

%Industrial wireless sensor networks play a vital role in smart industries integrated with Industry 4.0 framework. For ensuring better data quality and better communication services in Industrial wireless sensor networks, Li et al.\cite{li_review_2017} proposed new architecture that tailors the networks for ubiquitous industrial communication applications. Transformation towards wireless factory is developed using a graphical model\cite{candell_sysml_2019}, that employs Systems Modeling Language for identifying the behaviors, interfaces, and structural features of wireless networks with analyzes on the delay, data loss and data flows.\par

%IIoT data flow and communication depending on condition-based maintenance are formulated using a learning algorithm\cite{koulali_industrial_2018}, developed to maintain the health rate of equipment under surveillance using mean-field equilibrium. Application driven networks are used to provide Dynamic Data Distribution Service for enabling the efficiency standards for IIoT communication services\cite{abdellatif_management_2020}. Moreover, bit error rates are improved in the communication between smart machines in smart industries using convolutional codes and reed-Solomon codes\cite{saadaoui_improved_2020}.

%------------------------------------------------------------------------------
\subsubsection{Trustworthiness of IIoT Data in Smart Manufacturing}

With the adoption of connected systems in the manufacturing process, we also face increasing cybersecurity risks. So, an adaptation of Industry 4.0 requires close collaboration of Information Technology (IT) experts for the implementation of cybersecurity with the best aspects across the digital ecosystem to enhance the privacy and security features. To this aim, several efforts have been made. For instance, trust between humans and machines is enforced using cyber-physical-human analysis\cite{jiao_towards_2020}, that enhances the trust in dynamic modeling, cognitive prediction and optimized interaction between humans and machines. Some of the major security threats faced by IIoT devices/machines are shown in Fig. \ref{fig:IIoTthreats}. Similarly, Hehenberger et al.\cite{hehenberger_design_2016} reviewed the mechatronics systems in the industries and their transition towards secured Cyber-physical systems and cloud-based IIoT systems. Secure Blockchain Tokenizer is also used for securing IIoT data collected from the supply chain in smart industries\cite{mazzei_blockchain_2020}. Data acquisition, monitoring, and teleoperation of IIoT data from CNC machines are performed using the architecture developed using an internet-based client-server model through the web systems\cite{alvares_development_2018}. The developed CyberDNC web systems are validated with a focus on secured connectivity between the servers and the CNC machines. \par

Moreover, MCloud platform was developed by Lu et al.\cite{lu_energy-efficient_2019} for establishing a secure and energy-efficient production network with improved privacy features and enhanced flexibility in the Industry 4.0 environment. The framework was also used for collaborative energy-efficient manufacturing for distributed manufacturers to coordinate production processes that are customized based on requirements. In\cite{liu_industrial_2020}, the researchers developed an industrial blockchain-based product lifecycle management model for the exchange of secure data services, secured storage platform, decentralized data access, and interoperability among Industry 4.0 compatible networks. IIoT based data-driven security enforcement is also applied to circuit breaker production\cite{chen_framework_2020} in smart factories. However, trustworthiness of IIoT devices/machines can be ensured by carefully addressing the 5 pillars of trustworthiness of IIoT devices as shown in Fig. \ref{fig:IIoTpillars}. \par
%------------------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
  \centering    
  \includegraphics[width=0.45\textwidth]{figures/3.png}
  \caption{The 5 pillars of trustworthiness towards IIoT devices / machines.}
     \label{fig:IIoTpillars}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[!ht]
%  \centering    
%  \includegraphics[width=0.48\textwidth]{figures/Data_Issues.png}
%  \caption{Data related issues hindering a successful deployment of AI in Industry 4.0}
%     \label{fig:data-related-issues}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------------------------------------------------------------
%\subsubsection{Cloud Services for IIoT Big data }

%A hybrid cloud-IoT model is proposed by at al.\cite{elhoseny_hybrid_2018} for handling big data from health care applications with integrated mechanisms towards the Industry 4.0 model of applications. The existing challenges in Cloud Manufacturing autonomy of machines under three different levels are effectively managed using proposed cloud-based business models for smart industries\cite{charro_cloud_2018}. Smart industries also demand cloud-assisted Cyber-Physical Systems that combine IoT, AI, big data, and cloud computing for information management among the data collected from the smart manufacturing devices\cite{wan_cloud-assisted_2017}. Cloud-based manufacturing providing services based on demand enabled using the Internet are established for making large transformations in the production processes\cite{lu_cloud-based_2019}. 
